Where Did Your Model Learn That? Label-free Influence for Self-supervised Learning

Self-supervised learning (SSL) has revolutionized learning from large-scale unlabeled datasets, yet the intrinsic relationship between pretraining data and the learned representations remains poorly understood. Traditional supervised learning benefits from gradient-based data attribution tools like influence functions that measure the contribution of an individual data point to model predictions. However, existing definitions of influence rely on labels, making them unsuitable for SSL settings. We address this gap by introducing Influence-SSL, a novel and label-free approach for defining influence functions tailored to SSL. Our method harnesses the stability of learned representations against data augmentations to identify training examples that help explain model predictions. We provide both theoretical foundations and empirical evidence to show the utility of Influence-SSL in analyzing pre-trained SSL models. Our analysis reveals notable differences in how SSL models respond to influential data compared to supervised models. Finally, we validate the effectiveness of Influence-SSL through applications in duplicate detection, outlier identification and fairness analysis. Code is available at: \url{https://github.com/cryptonymous9/Influence-SSL}.

==> sections/new_theory.tex <==
\amit{PBRF results}
\subsection{Proximal Bregman Response Functions}

As shown by Bae et al., influence functions in neural networks actually approximate the Proximal Bregman Response Function (PBRF):

\begin{align*}
    r^b_{\pm z,\text{damp}}(\epsilon) = &\arg\min_{\theta \in \mathbb{R}^d} \frac{1}{N}\sum_{i=1}^N D_L^{(i)}(f(\theta, x^{(i)}), f(\theta_s, x^{(i)})) \\  &\pm \epsilon L(f(\theta, x), t) + \frac{\lambda}{2}\|\theta - \theta_s\|^2
\end{align*}

where $D_L^{(i)}$ is the Bregman divergence:

\begin{equation}
    D_L^{(i)}(y, y_s) = L(y, t^{(i)}) - L(y_s, t^{(i)}) - \nabla_y L(y_s, t^{(i)})^T(y - y_s)
\end{equation}

This formulation addresses two key issues in applying influence functions to neural networks: non-uniqueness of optima in overparameterized settings and the practice of early stopping before convergence.

\subsection{Practical Approximations in Large Models}

Recent work by Grosse et al. has demonstrated several approximations necessary for scaling influence functions to large language models. 

For large neural networks, computing the exact inverse Hessian is computationally intractable, requiring $O(d^3)$ operations for $d$ parameters. The Eigenvalue-corrected Kronecker-Factored Approximate Curvature (EK-FAC) provides a structured approximation of the Gauss-Newton Hessian $G$. For a multilayer perceptron (MLP) layer with input dimension $M$ and output dimension $P$, the pre-activation outputs $s_\ell$ are computed as:

\begin{equation}
    s_\ell = W_\ell a_{\ell-1} + b_\ell
\end{equation}

where $W_\ell \in \mathbb{R}^{P \times M}$ is the weight matrix, $a_{\ell-1} \in \mathbb{R}^M$ are the input activations, and $b_\ell \in \mathbb{R}^P$ is the bias vector. Let us define the homogeneous coordinates $\bar{a}_{\ell-1} = [a_{\ell-1}^T, 1]^T$ and $\bar{W}_\ell = [W_\ell, b_\ell]$ for notational convenience.

The EK-FAC approximation assumes that the activations and pre-activation gradients are independent, leading to:

\begin{equation}
    G_\ell \approx \mathbb{E}[\bar{a}_{\ell-1}\bar{a}_{\ell-1}^T] \otimes \mathbb{E}[Ds_\ell Ds_\ell^T] = A_{\ell-1} \otimes S_\ell
\end{equation}

where $Ds_\ell = \nabla_{s_\ell} \log p(\hat{y}|\theta, x)$ represents the pre-activation pseudo-gradient, and $\otimes$ denotes the Kronecker product. The matrices $A_{\ell-1} \in \mathbb{R}^{(M+1) \times (M+1)}$ and $S_\ell \in \mathbb{R}^{P \times P}$ are uncentered covariance matrices of activations and pre-activation gradients respectively.

EK-FAC further refines this approximation by computing eigendecompositions:

\begin{equation}
    A_{\ell-1} = Q_A \Lambda_A Q_A^T, \quad S_\ell = Q_S \Lambda_S Q_S^T
\end{equation}

and fitting a more accurate diagonal approximation in the Kronecker-factored eigenbasis:

\begin{equation}
    G_\ell \approx (Q_A \otimes Q_S)\Lambda(Q_A \otimes Q_S)^T
\end{equation}

where $\Lambda$ is diagonal with entries:

\begin{equation}
    \Lambda_{ii} = \mathbb{E}[((Q_A \otimes Q_S)D\theta)_i^2]
\end{equation}

This structure allows efficient computation of matrix operations while capturing important curvature information.

To further reduce computational costs, a block-diagonal structure is imposed across layers:

\begin{equation}
    G \approx \text{diag}(G_1, G_2, ..., G_L)
\end{equation}

This approximation assumes independence between parameter updates in different layers, which, while not strictly true, often works well in practice due to the hierarchical nature of neural networks.

Finally, for handling multiple influence queries efficiently, the preconditioned query gradients are approximated with rank $r$ approximations:

\begin{equation}
    v_q = (G + \lambda I)^{-1}\nabla_\theta f(\theta_s) \approx UV^T
\end{equation}

where $U,V \in \mathbb{R}^{d \times r}$. The rank $r$ is typically chosen much smaller than the dimension $d$, but large enough to capture the primary directions of influence.

\section{Analysis Framework}

\subsection{Modified Optimization Landscape}

These approximations fundamentally alter the optimization landscape of the influence computation where the influence functions presumably may not model the PBRF accurately any more. We begin by analyzing how the EK-FAC approximation modifies the optimization landscape. The Kronecker factorization introduces structural assumptions about parameter interactions, leading to a modified objective:

\begin{align*}
    \min_\theta \frac{1}{N}&\sum_{i=1}^N D_L^{(i)}(f(\theta, x^{(i)}), f(\theta_s, x^{(i)})) \pm \epsilon L(f(\theta, x), t) \\
    &+ \frac{1}{2}(\theta - \theta_s)^T(G_{\text{EK-FAC}} + \lambda I)(\theta - \theta_s)
\end{align*}

where $G_{\text{EK-FAC}}$ has the Kronecker-factored structure. The block-diagonal approximation further decomposes this into layer-wise independent optimizations:

\begin{align*}
    \min_{\theta_1,...,\theta_L} \sum_{\ell=1}^L \left[&\frac{1}{N}\sum_{i=1}^N D_{L,\ell}^{(i)}(f_\ell(\theta_\ell, x^{(i)}), f_\ell(\theta_{s,\ell}, x^{(i)})) \\
    &\pm \epsilon L_\ell(f_\ell(\theta_\ell, x), t) \\
    &\left+ \frac{1}{2}(\theta_\ell - \theta_{s,\ell})^T(G_{\ell,\text{EK-FAC}} + \lambda I)(\theta_\ell - \theta_{s,\ell})\right]
\end{align*}

where $f_\ell$ denotes the computation up to layer $\ell$, and $D_{L,\ell}^{(i)}$ and $L_\ell$ represent the layer-wise decomposition of the Bregman divergence and loss respectively.

The low-rank gradient approximation effectively restricts the solution to lie in a reduced subspace:

\begin{equation}
    \theta - \theta_s = UV^T\alpha
\end{equation}

for some coefficient vector $\alpha \in \mathbb{R}^r$.

Intuitively, these approximations create a hierarchy of constraints on the parameter updates:
\begin{enumerate}
    \item The Kronecker factorization enforces a particular structure on parameter interactions within each layer.
    \item The block-diagonal approximation prevents information flow between layers during the influence computation.
    \item The low-rank approximation restricts updates to lie in a reduced subspace determined by the most important directions of influence.
\end{enumerate}

\amit{The resulting mathematical object I think can be viewed as a projection of the original PBRF onto this constrained space, where the projection is defined by the various approximation structures. So I'm thinking that the scaled influence functions are computing a kind of "structured PBRF".}



\subsection{Theoretical Analysis}

The key theoretical question is understanding how these approximations transform the optimization landscape and therefore the object being approximated. The Kronecker factorization introduces implicit independence assumptions between input and output dimensions within each layer. The block-diagonal structure assumes independence between layers. The low-rank approximations of gradients introduce a form of dimensionality reduction.

\amit{Conjecture: the resulting object can be characterized as a constrained version of the PBRF where parameter updates are restricted to lie in certain subspaces determined by the approximation structure. First, we need to derive explicit forms for the optimization problems at each approximation level. Second, we can analyze the geometric relationship between these approximations and the original PBRF to have nice interpretation and figures like the earlier papers of Grosse. Third, we should establish bounds on the approximation error introduced at each step. Right now, I am trying to start with simplified settings where exact computation is possible and gradually incorporate complexity.}


\section{Theoretical Analysis}
\label{sec:analysis}

Let us begin by establishing the necessary definitions and assumptions:

\begin{definition}[EK-FAC Response Function]
Given a neural network $f: \mathbb{R}^d \times \mathcal{X} \to \mathbb{R}^k$ parameterized by $\theta \in \mathbb{R}^d$, we define the EK-FAC modified response function as:
\begin{align}
    &r^b_{\text{EK-FAC}}(\epsilon) \\
    &= \arg\min_{\theta} \frac{1}{N}\sum_{i=1}^N D_L^{(i)}(f(\theta, x^{(i)}), f(\theta_s, x^{(i)})) \pm \epsilon L(f(\theta, x), t) \nonumber \\
    &+ \frac{1}{2}(\theta - \theta_s)^T((Q_A \otimes Q_S)\Lambda(Q_A \otimes Q_S)^T + \lambda I)(\theta - \theta_s)
\end{align}
where $Q_A$, $Q_S$ are orthogonal matrices and $\Lambda$ is diagonal.
\end{definition}

\begin{assumption}[Loss Convexity]
\label{assump:loss}
The loss function $L$ is twice continuously differentiable and strictly convex in its first argument.
\end{assumption}

\begin{assumption}[Network Smoothness]
\label{assump:smooth}
The network function $f(\theta, x)$ is twice continuously differentiable in $\theta$ with Lipschitz continuous gradients.
\end{assumption}

\begin{assumption}[EK-FAC Positive Definiteness]
\label{assump:ekfac}
The matrix $(Q_A \otimes Q_S)\Lambda(Q_A \otimes Q_S)^T + \lambda I$ is positive definite with minimum eigenvalue at least $\mu > 0$.
\end{assumption}


Our main theorem establishes that influence functions with EK-FAC approximation correspond to a first-order approximation of the EK-FAC response function:


\begin{theorem}[PBRF Approximation]
Let $r^b_{\pm z,\text{damp}}(\epsilon)$ be the original PBRF and $r^b_{\text{EK-FAC}}(\epsilon)$ be the EK-FAC modified version. Under Assumptions \ref{assump:loss}-\ref{assump:ekfac}, and assuming:

\begin{assumption}[Curvature Approximation Quality]
\label{assump:curvature}
$\|G - G_{\text{EK-FAC}}\| \leq \delta$ for some $\delta > 0$
\end{assumption}

\begin{assumption}[Gradient Lipschitz]
\label{assump:lipschitz}
The gradients of $f$ and $L$ are Lipschitz continuous with constants $L_f$ and $L_L$ respectively.
\end{assumption}

Then for sufficiently small $|\epsilon|$:
\begin{equation}
    \|r^b_{\text{EK-FAC}}(\epsilon) - r^b_{\pm z,\text{damp}}(\epsilon)\| \leq K\delta
\end{equation}
where $K$ depends on $L_f$, $L_L$, and $\lambda$.
\end{theorem}

\begin{proof}[Proof Sketch]

\amit{Incomplete proof idea}

The proof would proceed by:

1. Write the optimality conditions for both response functions:
\begin{align}
    \nabla_\theta \mathcal{L}_{\text{PBRF}}(r^b_{\pm z,\text{damp}}(\epsilon)) &= 0 \\
    \nabla_\theta \mathcal{L}_{\text{EK-FAC}}(r^b_{\text{EK-FAC}}(\epsilon)) &= 0
\end{align}

2. The difference in these gradients comes from the different proximity terms:
\begin{align}
    \nabla_\theta \mathcal{L}_{\text{PBRF}}(\theta) - \nabla_\theta \mathcal{L}_{\text{EK-FAC}}(\theta) 
    = (G - G_{\text{EK-FAC}})(\theta - \theta_s)
\end{align}

3. Use strong convexity and the assumed bound on $\|G - G_{\text{EK-FAC}}\|$ to bound the difference in the solutions.

However, this proof sketch has challenges:
- Need to carefully track how $\epsilon$ affects the bounds
- Must ensure strong convexity is uniform
- Need to handle the nonlinearity of $f$
\end{proof}

\subsection{Relationship to Original PBRF}

To understand how this modified response function relates to the original PBRF, we can establish:

\begin{theorem}[PBRF Approximation]
\label{thm:pbrf}
Under suitable conditions on the EK-FAC approximation quality:
\begin{equation}
    \|r^b_{\text{EK-FAC}}(\epsilon) - r^b_{\pm z,\text{damp}}(\epsilon)\| \leq K\|G - G_{\text{EK-FAC}}\|
\end{equation}
where $K$ is a problem-dependent constant and $G_{\text{EK-FAC}} = (Q_A \otimes Q_S)\Lambda(Q_A \otimes Q_S)^T$.
\end{theorem}

\amit{Still need to prove this}




\section{PBRF and SSL-Influence}

Recent work has shown that while influence functions are widely used to approximate leave-one-out retraining in deep networks, they actually approximate a different quantity called the Proximal Bregman Response Function (PBRF). However, existing theory for influence functions assumes access to labeled data, making it unsuitable for self-supervised learning (SSL) settings. In this section, we extend the PBRF framework to handle pairs of augmented views in SSL, providing a principled way to understand what influence functions approximate in self-supervised learning.

\subsection{Preliminaries and Notation}

Let $f_\theta: \mathcal{X} \to \mathbb{R}^d$ denote an encoder network parameterized by $\theta \in \mathbb{R}^p$. In the SSL setting, each input $x \in \mathcal{X}$ is paired with an augmented view $\hat{x}$. The relationship between these views is captured through cosine similarity:

\begin{equation}
    \text{sim}(a,b) = \frac{a^\top b}{\|a\| \|b\|}
\end{equation}

Following standard practice in SSL, we define the loss between an input and its augmented view as the negative cosine similarity plus one:

\begin{equation}
    L(f_\theta(x), f_\theta(\hat{x})) = 1 - \text{sim}(f_\theta(x), f_\theta(\hat{x}))
\end{equation}

\amit{Caveat: I have assumed a fixed augmentation which is not what we do but extending to stochastic augmentations introduces a sampling step here and is harder to analyze. Still thinking on how to do it.}

Given a dataset $\mathcal{D} = \{(x_i, \hat{x}_i)\}_{i=1}^N$ of input-augmentation pairs, the total empirical risk minimized during training is:

\begin{equation}
    J(\theta) = \frac{1}{N} \sum_{i=1}^N L(f_\theta(x_i), f_\theta(\hat{x}_i))
\end{equation}

\subsection{SSL Proximal Bregman Response Function}

To understand what influence functions actually approximate in SSL, we introduce the SSL Proximal Bregman Response Function (SSL-PBRF). For removing an example $z = (x_z, \hat{x}_z)$ from the training set, the SSL-PBRF is defined as:

\begin{equation}
\begin{split}
    &r^b_{-z}(\epsilon) \\
    &= \argmin_\theta \Big[  \frac{1}{N} \sum_{i=1}^N D_L(f_\theta(x_i), f_\theta(\hat{x}_i), f_{\theta_s}(x_i), f_{\theta_s}(\hat{x}_i)) \\
    & - \epsilon L(f_\theta(x_z), f_\theta(\hat{x}_z)) + \frac{\lambda}{2}\|\theta - \theta_s\|^2 \Big]
\end{split}
\end{equation}

where $\theta_s$ represents the current model parameters, $\lambda > 0$ is a damping parameter, and $D_L$ is the Bregman divergence defined as:

\begin{equation}
\begin{split}
    D_L(y_1,\hat{y}_1,y_2,\hat{y}_2) = & L(y_1,\hat{y}_1) - L(y_2,\hat{y}_2) \\
    & - \nabla_y L(y_2,\hat{y}_2)^\top(y_1-y_2) \\
    & - \nabla_{\hat{y}} L(y_2,\hat{y}_2)^\top(\hat{y}_1-\hat{y}_2)
\end{split}
\end{equation}

The SSL-PBRF objective serves three purposes. First, through the Bregman divergence terms, it encourages the new parameters to maintain similar view-consistency behavior to $\theta_s$ on the remaining examples. Second, it removes the influence of example $z$ through the negative loss term. Third, the proximity term $\frac{\lambda}{2}\|\theta - \theta_s\|^2$ ensures the new parameters stay close to $\theta_s$ in parameter space.

\subsection{Theoretical Analysis}

We now establish the theoretical foundations for understanding how influence functions relate to the SSL-PBRF. Our analysis begins by proving key properties of the SSL loss and its associated Bregman divergence, which are essential for the main result.

\begin{lemma}[Local Smoothness of SSL Loss]
For fixed $x,\hat{x}$, the function $L(f_\theta(x), f_\theta(\hat{x}))$ is $\beta$-smooth in a neighborhood of any point where both $\|f_\theta(x)\|$ and $\|f_\theta(\hat{x})\|$ are bounded away from zero.
\end{lemma}

\begin{proof}
Consider the SSL loss $L(f_\theta(x), f_\theta(\hat{x})) = 1 - \frac{f_\theta(x)^\top f_\theta(\hat{x})}{\|f_\theta(x)\| \|f_\theta(\hat{x})\|}$. 

In any neighborhood where both $\|f_\theta(x)\|$ and $\|f_\theta(\hat{x})\|$ are bounded away from zero, say by some constant $c > 0$, the denominator satisfies $\|f_\theta(x)\| \|f_\theta(\hat{x})\| \geq c^2 > 0$.

The numerator $f_\theta(x)^\top f_\theta(\hat{x})$ is smooth as a function of $\theta$ since $f_\theta$ is assumed to be smooth. The denominator is also smooth in this neighborhood since it is bounded away from zero and composed of smooth functions.

The quotient of smooth functions is smooth when the denominator is bounded away from zero. Therefore, there exists some $\beta > 0$ such that:

\begin{equation}
    \|\nabla_\theta L(f_{\theta_1}(x), f_{\theta_1}(\hat{x})) - \nabla_\theta L(f_{\theta_2}(x), f_{\theta_2}(\hat{x}))\| \leq \beta\|\theta_1 - \theta_2\|
\end{equation}

for all $\theta_1, \theta_2$ in this neighborhood.
\end{proof}

\begin{lemma}[Properties of SSL Bregman Divergence]
The Bregman divergence $D_L$ as defined for the SSL loss satisfies:
\begin{enumerate}
\item Non-negativity: $D_L(y_1,\hat{y}_1,y_2,\hat{y}_2) \geq 0$
\item Identity of indiscernibles: $D_L(y_1,\hat{y}_1,y_2,\hat{y}_2) = 0$ if and only if $y_1=y_2$ and $\hat{y}_1=\hat{y}_2$
\end{enumerate}
\end{lemma}

\begin{proof}
The proof follows from the local smoothness of $L$ established in Lemma 1. The Bregman divergence represents the difference between the function value and its first-order approximation at another point:

\begin{equation}
\begin{split}
    D_L(y_1,\hat{y}_1,y_2,\hat{y}_2) = & L(y_1,\hat{y}_1) - L(y_2,\hat{y}_2) \\
    & - \nabla_y L(y_2,\hat{y}_2)^\top(y_1-y_2) \\
    & - \nabla_{\hat{y}} L(y_2,\hat{y}_2)^\top(\hat{y}_1-\hat{y}_2)
\end{split}
\end{equation}

In regions where the loss is smooth, this difference is always non-negative and equals zero only when the points coincide. The gradient terms capture the full differential structure of the SSL loss with respect to both original and augmented views.
\end{proof}

These lemmas establish properties that ensure the SSL-PBRF objective is well-behaved. The local smoothness of the SSL loss in regions where network outputs have non-zero norm means that local approximations used in influence estimation are meaningful, while the Bregman divergence properties ensure that our objective properly captures discrepancies between different parameter settings.

We now present our main theoretical result connecting influence functions to the SSL-PBRF:

\begin{theorem}[SSL-PBRF First-Order Approximation]
Under assumptions A1-A3 below, the influence function estimation with damping parameter $\lambda > 0$:

\begin{equation}
\begin{split}
    I(f,z) =  -&\nabla_\theta L(f_{\theta_s}(x_z), f_{\theta_s}(\hat{x}_z))^\top (H_\theta + \lambda I)^{-1} \\
                &\nabla_\theta L(f_{\theta_s}(x_z), f_{\theta_s}(\hat{x}_z))
\end{split}
\end{equation}

where $H_\theta = \frac{1}{N} \sum_{i=1}^N \nabla^2_\theta L(f_{\theta_s}(x_i), f_{\theta_s}(\hat{x}_i))$, is equivalent to the first-order approximation of the SSL-PBRF at $\epsilon=0$.
\end{theorem}

The following assumptions are required for our analysis:

A1. The network $f_\theta$ is twice continuously differentiable with respect to $\theta$. This ensures the existence and continuity of all required derivatives in our analysis.

A2. The Hessian $H_\theta + \lambda I$ is positive definite at $\theta_s$. This assumption, combined with the damping term $\lambda I$, guarantees that our optimization problem is locally well-conditioned.

A3. The network outputs maintain non-zero norms during training, ensuring we remain in the regime where the SSL loss is locally smooth.

\begin{proof}
The proof proceeds by carefully analyzing the SSL-PBRF objective and its derivatives. 

Consider the objective for removing example $z$:

\begin{equation}
\begin{split}
    Q_z(\theta,\epsilon) = & \frac{1}{N} \sum_{i=1}^N D_L(f_\theta(x_i), f_\theta(\hat{x}_i), f_{\theta_s}(x_i), f_{\theta_s}(\hat{x}_i)) \\
    & - \epsilon L(f_\theta(x_z), f_\theta(\hat{x}_z)) + \frac{\lambda}{2}\|\theta - \theta_s\|^2
\end{split}
\end{equation}

First, we verify that at $\epsilon=0$, $\theta_s$ minimizes $Q_z(\theta,0)$. For the Bregman terms, $D_L(f_{\theta_s}(x_i), f_{\theta_s}(\hat{x}_i), f_{\theta_s}(x_i), f_{\theta_s}(\hat{x}_i)) = 0$ by Lemma 2, and the proximity term is clearly minimized at $\theta = \theta_s$.

Next, by the Implicit Function Theorem (which applies due to assumptions A1-A3), there exists a unique continuously differentiable function $r^b_{-z}(\epsilon)$ in a neighborhood of $\epsilon=0$ satisfying:

\begin{equation}
    \nabla_\theta Q_z(r^b_{-z}(\epsilon),\epsilon) = 0
\end{equation}

Taking the total derivative with respect to $\epsilon$:

\begin{equation}
    \nabla^2_\theta Q_z(r^b_{-z}(\epsilon),\epsilon) \cdot \frac{dr^b_{-z}}{d\epsilon} + \nabla^2_{\theta,\epsilon} Q_z(r^b_{-z}(\epsilon),\epsilon) = 0
\end{equation}

At $\epsilon=0$, this becomes:

\begin{equation}
    \nabla^2_\theta Q_z(\theta_s,0) \cdot \frac{dr^b_{-z}}{d\epsilon}\Big|_{\epsilon=0} = \nabla_\theta L(f_{\theta_s}(x_z), f_{\theta_s}(\hat{x}_z))
\end{equation}

Computing the Hessian $\nabla^2_\theta Q_z(\theta_s,0)$:

From the Bregman terms: $H_\theta = \frac{1}{N} \sum_{i=1}^N \nabla^2_\theta L(f_{\theta_s}(x_i), f_{\theta_s}(\hat{x}_i))$
From the proximity term: $\lambda I$

Therefore:

\begin{equation}
    \nabla^2_\theta Q_z(\theta_s,0) = H_\theta + \lambda I
\end{equation}

Solving for the derivative:

\begin{equation}
    \frac{dr^b_{-z}}{d\epsilon}\Big|_{\epsilon=0} = -(H_\theta + \lambda I)^{-1} \nabla_\theta L(f_{\theta_s}(x_z), f_{\theta_s}(\hat{x}_z))
\end{equation}

To connect this to the influence function formula in the theorem statement, we note that by the definition of influence functions, the predicted effect on any function $g(\theta)$ of removing example $z$ is given by:

\begin{equation}
    I_g(f,z) = \frac{dr^b_{-z}}{d\epsilon}\Big|_{\epsilon=0} \cdot \nabla_\theta g(\theta_s)
\end{equation}

In particular, when $g(\theta) = L(f_\theta(x_z), f_\theta(\hat{x}_z))$, we have:

\begin{equation}
\begin{split}
    I(f,z) &= \frac{dr^b_{-z}}{d\epsilon}\Big|_{\epsilon=0} \cdot \nabla_\theta L(f_{\theta_s}(x_z), f_{\theta_s}(\hat{x}_z)) \\
    &= -(H_\theta + \lambda I)^{-1} \nabla_\theta L(f_{\theta_s}(x_z), f_{\theta_s}(\hat{x}_z)) \cdot \nabla_\theta L(f_{\theta_s}(x_z), f_{\theta_s}(\hat{x}_z)) \\
    &= -\nabla_\theta L(f_{\theta_s}(x_z), f_{\theta_s}(\hat{x}_z))^\top (H_\theta + \lambda I)^{-1} \nabla_\theta L(f_{\theta_s}(x_z), f_{\theta_s}(\hat{x}_z))
\end{split}
\end{equation}

This matches exactly the influence function formula stated in the theorem, completing the proof.

\end{proof}

This result has important implications for understanding influence functions in SSL. While influence functions have been shown to not accurately track leave-one-out retraining in the supervised setting, they do provide first-order approximations to the PBRF. Our result extends this connection to the SSL setting, providing a principled way to evaluate influence estimations in self-supervised learning. The key insight is that while the SSL loss is not convex, it possesses sufficient smoothness properties in the regions where neural networks typically operate, allowing the influence function machinery to provide meaningful approximations to the SSL-PBRF.

\amit{We can actually try to prove some thing related to memorization. For a training example x with augmented view T(x), the memorization M(x) is approximated by the self-influence: M(x) = I(f,(x,T(x))) + O(epsilon) where I(f,(x,T(x))) is the SSL influence function we defined. What do you think? this might be able to connect the ssl-pbrf with memorization via leave one out loss. Might be possible depending on the right definition of M(x).}






\section{Extension to Stochastic Augmentations}

While our previous analysis assumed fixed augmentations, self-supervised learning methods typically employ stochastic augmentation strategies. In this section, we extend our theoretical framework to handle random augmentations, showing that influence functions still provide accurate approximations to a stochastic version of the SSL-PBRF.

\subsection{Stochastic SSL Framework}

Let $(\mathcal{H}, \mathcal{F}, P)$ be a probability space, where $\eta \sim P$ represents random parameters controlling the augmentation process. 

The augmentation function $T: \mathcal{X} \times \mathcal{H} \to \mathcal{X}$ maps an input $x$ and random parameters $\eta$ to an augmented view $T(x,\eta)$. This formulation captures common augmentation strategies such as random crops, color jittering, and Gaussian blur, where $\eta$ determines the specific transformation applied.

For an input $x$ and parameters $\theta$, we define the expected SSL loss:
\begin{equation}
    \mathcal{L}(f_\theta, x) = \mathbb{E}_{\eta \sim P}[L(f_\theta(x), f_\theta(T(x,\eta)))]
\end{equation}

\amit{Note: I haven't assumed that P is a discrete set (i.e. fixed set of augmentations). The rpoof still seems to go through.}

where $L$ remains the cosine distance between representations as before. The total empirical risk becomes:
\begin{equation}
    J(\theta) = \frac{1}{N} \sum_{i=1}^N \mathbb{E}_{\eta \sim P}[L(f_\theta(x_i), f_\theta(T(x_i,\eta)))]
\end{equation}

To analyze this stochastic setting, we require several technical assumptions:

A1. The encoder network $f_\theta$ is twice continuously differentiable with respect to $\theta$. This ensures the existence of required derivatives and enables application of the Implicit Function Theorem.

A2. For any fixed $x$ and $\eta$, the augmentation $T(x,\eta)$ is measurable and the loss $L(f_\theta(x), f_\theta(T(x,\eta)))$ is bounded when network outputs have non-zero norm. This allows proper definition of expectations and ensures finite losses.

A3. The derivatives of the loss with respect to parameters are uniformly bounded across augmentations in regions where network outputs maintain non-zero norm:
\begin{equation}
    \sup_{\eta} \|\nabla_\theta L(f_\theta(x), f_\theta(T(x,\eta)))\| \leq M_1
\end{equation}
\begin{equation}
    \sup_{\eta} \|\nabla^2_\theta L(f_\theta(x), f_\theta(T(x,\eta)))\| \leq M_2
\end{equation}

A4. The network outputs maintain non-zero norms during training, ensuring we remain in the regime where the SSL loss is locally smooth.

A5. The expected Hessian with damping, $\mathcal{H}_\theta + \lambda I$ where
\begin{equation}
    \mathcal{H}_\theta = \mathbb{E}_\eta[\nabla^2_\theta L(f_\theta(x), f_\theta(T(x,\eta)))]
\end{equation}
is positive definite at $\theta_s$.

\subsection{Local Smoothness in the Stochastic Setting}

Before proceeding to the main result, we establish the smoothness properties of the expected SSL loss:

\begin{lemma}[Local Smoothness of Expected SSL Loss]
Under assumptions A1-A4, for fixed $x$, the expected loss $\mathcal{L}(f_\theta, x)$ is $\beta$-smooth in a neighborhood of any point where network outputs maintain non-zero norm.
\end{lemma}

\begin{proof}
By assumption A4, we operate in a region where network outputs have non-zero norm. In this region, we established in our previous analysis that the SSL loss is locally smooth for any fixed augmentation. The uniform boundedness of derivatives (A3) allows us to extend this to the expected loss via the dominated convergence theorem:

\begin{equation}
\begin{split}
    \|\nabla_\theta \mathcal{L}(f_{\theta_1}, x) - \nabla_\theta \mathcal{L}(f_{\theta_2}, x)\| &= \|\mathbb{E}_\eta[\nabla_\theta L(f_{\theta_1}, T) - \nabla_\theta L(f_{\theta_2}, T)]\| \\
    &\leq \mathbb{E}_\eta[\|\nabla_\theta L(f_{\theta_1}, T) - \nabla_\theta L(f_{\theta_2}, T)\|] \\
    &\leq \beta\|\theta_1 - \theta_2\|
\end{split}
\end{equation}

where we use $T$ as shorthand for $T(x,\eta)$ and the final inequality follows from the smoothness of the SSL loss for each fixed augmentation.
\end{proof}

\subsection{Stochastic SSL-PBRF}

We now define the stochastic SSL-PBRF for removing example $z$ as:
\begin{equation}
\begin{split}
&r^b_{-z}(\epsilon) \\
&= \argmin_\theta \Big[ \frac{1}{N} \sum_{i=1}^N \mathbb{E}_\eta[D_L(f_\theta(x_i), f_\theta(T(x_i,\eta)), f_{\theta_s}(x_i), f_{\theta_s}(T(x_i,\eta)))] \\
& - \epsilon \mathbb{E}_\eta[L(f_\theta(x_z), f_\theta(T(x_z,\eta)))] + \frac{\lambda}{2}\|\theta - \theta_s\|^2 \Big]
\end{split}
\end{equation}

This objective extends our previous SSL-PBRF by taking expectations over random augmentations. The Bregman divergence terms now encourage consistency with $\theta_s$ across all possible augmentations, while the second term removes the influence of example $z$ averaged over its augmented views.

\begin{theorem}[Stochastic SSL-PBRF First-Order Approximation]
Under assumptions A1-A5, the expected influence function:
\begin{equation}
\begin{split}
    I(f,z) = -&\mathbb{E}_\eta[\nabla_\theta L(f_{\theta_s}(x_z), f_{\theta_s}(T(x_z,\eta)))^\top] (\mathcal{H}_\theta + \lambda I)^{-1} \\  &\mathbb{E}_\eta[\nabla_\theta L(f_{\theta_s}(x_z), f_{\theta_s}(T(x_z,\eta)))]
\end{split}
\end{equation}
is equivalent to the first-order approximation of the stochastic SSL-PBRF at $\epsilon=0$.
\end{theorem}

\begin{proof}
Let $Q_z(\theta,\epsilon)$ denote the stochastic SSL-PBRF objective. The uniform boundedness conditions in A3 allow us to exchange expectation and differentiation via the Dominated Convergence Theorem:
\begin{equation}
    \nabla_\theta \mathbb{E}_\eta[L(f_\theta(x), f_\theta(T(x,\eta)))] = \mathbb{E}_\eta[\nabla_\theta L(f_\theta(x), f_\theta(T(x,\eta)))]
\end{equation}

\amit{The above technical step is where we require the bounded gradients assumption}

At $\epsilon=0$, $\theta_s$ minimizes $Q_z(\theta,0)$ since both the expected Bregman divergence terms and proximity term achieve their minimum at $\theta_s$. This follows from the local smoothness established in our lemma and the properties of Bregman divergences.

By the Implicit Function Theorem (which applies due to A1 and A5), there exists a unique continuously differentiable function $r^b_{-z}(\epsilon)$ in a neighborhood of $\epsilon=0$ satisfying:

\begin{equation}
    \nabla_\theta Q_z(r^b_{-z}(\epsilon),\epsilon) = 0
\end{equation}

Taking the total derivative with respect to $\epsilon$ and evaluating at $\epsilon=0$:
\begin{equation}
    \nabla^2_\theta Q_z(\theta_s,0) \cdot \frac{dr^b_{-z}}{d\epsilon}\Big|_{\epsilon=0} = \mathbb{E}_\eta[\nabla_\theta L(f_{\theta_s}(x_z), f_{\theta_s}(T(x_z,\eta)))]
\end{equation}

The Hessian $\nabla^2_\theta Q_z(\theta_s,0)$ equals $\mathcal{H}_\theta + \lambda I$, where the expectation over augmentations arises from differentiating the Bregman terms and the $\lambda I$ comes from the proximity regularization. Therefore:
\begin{equation}
    \frac{dr^b_{-z}}{d\epsilon}\Big|_{\epsilon=0} = -(\mathcal{H}_\theta + \lambda I)^{-1} \mathbb{E}_\eta[\nabla_\theta L(f_{\theta_s}(x_z), f_{\theta_s}(T(x_z,\eta)))]
\end{equation}

Following the same chain of reasoning as in the fixed augmentation case, this derivative exactly matches our expected influence function formula, completing the proof.
\end{proof}

This result extends our previous analysis to show that influence functions remain valid approximations even with stochastic augmentations, provided we properly account for expectations over the augmentation distribution. The key insight is that while the SSL loss is not convex, it maintains sufficient smoothness properties in regions where network outputs have non-zero norm. This smoothness, combined with the boundedness of derivatives across augmentations, allows the influence function machinery to provide meaningful approximations to the stochastic SSL-PBRF.




\section{Generalization to Abstract SSL Losses}

\amit{Need to verify these properties. Basically the idea here is what can we replace the cosine distance with and still get a connection to pbrf?}

While our previous analysis focused on cosine distance as the similarity measure between augmented views, self-supervised learning employs diverse loss functions. In this section, we show that our theoretical framework extends naturally to a broad class of SSL losses, encompassing many commonly used objectives in practice. This generalization reveals fundamental properties about influence functions in self-supervised learning that transcend specific architectural or loss choices.


\subsection{Abstract SSL Loss Functions}

We begin by defining the essential properties required of an SSL loss function for our analysis to hold. Rather than requiring convexity, which is too strong for typical SSL losses, we establish conditions ensuring sufficient local smoothness and boundedness.

\begin{definition}[Admissible SSL Loss]
A function $\mathcal{L}: \mathbb{R}^d \times \mathbb{R}^d \to \mathbb{R}$ is an admissible SSL loss if for some constants $c, M_1, M_2 > 0$, it satisfies:

\begin{equation}
    \text{(i) } \mathcal{L} \text{ is twice continuously differentiable in both arguments on } \Omega_c
\end{equation}

\begin{equation}
    \text{(ii) } \|\nabla_x \mathcal{L}(x,y)\| \leq M_1 \text{ for all } (x,y) \in \Omega_c
\end{equation}

\begin{equation}
    \text{(iii) } \|\nabla^2_x \mathcal{L}(x,y)\| \leq M_2 \text{ for all } (x,y) \in \Omega_c
\end{equation}

where $\Omega_c = \{(x,y) : \|x\|, \|y\| \geq c\}$ is the domain where representations have norm at least $c$.
\end{definition}

These conditions ensure the loss function is sufficiently well-behaved in regions where network outputs have non-zero norm, which is the typical case during training. We now show that common SSL losses satisfy these requirements:

\begin{proposition}[Cosine Distance]
The normalized cosine distance $\mathcal{L}_{\text{cos}}(x,y) = 1 - \frac{x^\top y}{\|x\|\|y\|}$ is an admissible SSL loss.
\end{proposition}

\begin{proof}
Fix $c > 0$ and consider $(x,y) \in \Omega_c$. First, we verify twice differentiability. The gradient with respect to x is:
\begin{equation}
    \nabla_x \mathcal{L}_{\text{cos}}(x,y) = -\frac{y}{\|x\|\|y\|} + \frac{x^\top y}{\|x\|^3\|y\|}x
\end{equation}

The Hessian is:
\begin{equation}
    \nabla^2_x \mathcal{L}_{\text{cos}}(x,y) = \frac{x^\top y}{\|x\|^3\|y\|}I + \frac{3(x^\top y)}{\|x\|^5\|y\|}xx^\top - \frac{1}{\|x\|^3\|y\|}(xy^\top + yx^\top)
\end{equation}

Since $\|x\|, \|y\| \geq c$, we have:
\begin{equation}
    \|\nabla_x \mathcal{L}_{\text{cos}}(x,y)\| \leq \frac{1}{c} + \frac{1}{c} = \frac{2}{c} = M_1
\end{equation}

For the Hessian norm, using the triangle inequality and Cauchy-Schwarz:
\begin{equation}
    \|\nabla^2_x \mathcal{L}_{\text{cos}}(x,y)\| \leq \frac{4}{c^3} = M_2
\end{equation}

Therefore, $\mathcal{L}_{\text{cos}}$ satisfies all conditions of admissibility.
\end{proof}

\begin{proposition}[InfoNCE Loss]
The InfoNCE loss with temperature $\tau > 0$:
\begin{equation}
    \mathcal{L}_{\text{NCE}}(x,y) = -\log\frac{\exp(x^\top y/\tau)}{\sum_{i=1}^N \exp(x^\top y_i/\tau)}
\end{equation}
is admissible when restricted to normalized inputs $\|x\| = \|y\| = 1$.
\end{proposition}

\begin{proof}
On the unit sphere, $|x^\top y| \leq 1$ by Cauchy-Schwarz, ensuring the exponential terms are bounded. The gradient involves terms of form $\exp(x^\top y/\tau)/\sum_i \exp(x^\top y_i/\tau)$, which are bounded between 0 and 1. The Hessian involves second derivatives of softmax, which are also bounded on this compact domain. Therefore, there exist constants $M_1, M_2$ satisfying the admissibility conditions.
\end{proof}

\begin{proposition}[BYOL Loss]
The BYOL loss $\mathcal{L}_{\text{BYOL}}(x,y) = \|x - \text{sg}(y)\|^2$, where $\text{sg}$ denotes stop-gradient, is an admissible SSL loss when restricted to any bounded domain.
\end{proposition}

\begin{proof}
With stop-gradient, $y$ is treated as a constant, making this equivalent to a squared Euclidean distance to a fixed point. On any bounded domain $\|x\|, \|y\| \leq R$, the gradient $2(x-y)$ has norm bounded by $4R$, and the Hessian $2I$ has constant norm 2, satisfying admissibility.
\end{proof}

\begin{proposition}[VICReg Invariance Term]
The VICReg invariance loss $\mathcal{L}_{\text{VIC}}(x,y) = \|x - y\|^2$ is an admissible SSL loss when restricted to any bounded domain.
\end{proposition}

\begin{proof}
On any bounded domain $\|x\|, \|y\| \leq R$, the gradient $2(x-y)$ and Hessian $2I$ satisfy the same bounds as the BYOL loss, establishing admissibility.
\end{proof}

\begin{proposition}[DINO Cross-Entropy]
The DINO loss with teacher network $g$:
\begin{equation}
    \mathcal{L}_{\text{DINO}}(x,y) = -\sum_i g(y)_i \log(\text{softmax}(x)_i)
\end{equation}
is admissible when the teacher outputs are bounded away from 0 and 1 and inputs are bounded.
\end{proposition}

\begin{proof}
When teacher outputs are bounded away from 0 and 1 by some $\delta > 0$ and inputs are bounded by $R$, the gradient and Hessian of the cross-entropy with respect to logits are bounded. The specific bounds depend on $\delta$ and $R$ but are finite, satisfying admissibility.
\end{proof}

With these properties established, we can state our main result for general SSL losses:

\begin{theorem}[General SSL-PBRF First-Order Approximation]
Let $\mathcal{L}$ be an admissible SSL loss. Under assumptions A1-A5, the expected influence function with general loss $\mathcal{L}$:
\begin{equation}
    I_{\mathcal{L}}(f,z) = -\mathbb{E}_\eta[\nabla_\theta \mathcal{L}(f_{\theta_s}(x_z), f_{\theta_s}(T(x_z,\eta)))^\top] (\mathcal{H}_{\mathcal{L},\theta} + \lambda I)^{-1} \mathbb{E}_\eta[\nabla_\theta \mathcal{L}(f_{\theta_s}(x_z), f_{\theta_s}(T(x_z,\eta)))]
\end{equation}
where
\begin{equation}
    \mathcal{H}_{\mathcal{L},\theta} = \frac{1}{N} \sum_{i=1}^N \mathbb{E}_\eta[\nabla^2_\theta \mathcal{L}(f_{\theta_s}(x_i), f_{\theta_s}(T(x_i,\eta)))]
\end{equation}
is equivalent to the first-order approximation of the general SSL-PBRF at $\epsilon=0$.
\end{theorem}

The proof follows the same structure as our earlier analysis of the cosine distance case, relying on the local smoothness and boundedness guaranteed by admissibility rather than convexity.

This generalization reveals several important insights about influence in self-supervised learning. First, it shows that the approximation properties of influence functions are fundamental to SSL, not artifacts of particular loss choices. Second, our admissibility conditions identify the key mathematical properties needed for reliable influence estimation across different SSL methods. Finally, these conditions align with properties that typically promote stable SSL training, suggesting that well-behaved influence functions might naturally emerge from good SSL loss design.

The framework also provides clear guidance for analyzing new SSL losses: if they satisfy our admissibility conditions on an appropriate domain, they automatically inherit all the influence function properties we have established. This enables systematic evaluation of influence estimation for novel SSL methods without requiring case-by-case analysis.

\amit{The above is what I think. not sure if what I'm claiming is too strong.}

\section{Additivity}






\amit{Connection with geometry}
\section{Relationship Between Influence and Representation Geometry}

\subsection{Setup}

Let $f_\theta: \mathcal{X} \to \mathbb{R}^d$ be an encoder network with parameters $\theta$. The SSL loss for an input $x$ is:

\begin{equation}
    L_{\text{ssl}}(\theta,x) = 1 - \cos(f_\theta(x), f_\theta(T(x)))
\end{equation}

where $\cos(a,b) = \frac{a^T b}{\|a\| \|b\|}$ and $T$ is a deterministic augmentation.

The influence function for point $x$ is:
\begin{equation}
    I(x) = -\nabla_\theta L_{\text{ssl}}(\theta,x)^T H^{-1} \nabla_\theta L_{\text{ssl}}(\theta,x)
\end{equation}

where $H = \mathbb{E}_{x}[\nabla^2_\theta L_{\text{ssl}}(\theta,x)]$ is the Hessian.

For any $x$, define its $\epsilon$-neighborhood in representation space:
\begin{equation}
    S_\epsilon(x) = \{y \in \mathcal{X}: \|f_\theta(y) - f_\theta(x)\| < \epsilon\}
\end{equation}

\subsection{Assumptions}

\begin{enumerate}[label=(A\arabic*)]
    \item $f_\theta$ is $\beta$-smooth: For all $x,y \in \mathcal{X}$,
          \[\|\nabla f_\theta(x) - \nabla f_\theta(y)\| \leq \beta\|x-y\|\]
    \item Representations are normalized: For all $x \in \mathcal{X}$,
          \[\|f_\theta(x)\| = 1\]
    \item $H$ is symmetric positive definite with bounded eigenvalues:
          \[0 < \lambda_{\min}(H) \leq \lambda_{\max}(H) < \infty\]
    \item $T$ is $(1+\delta)$-Lipschitz: For all $x,y \in \mathcal{X}$,
          \[\|T(x) - T(y)\| \leq (1+\delta)\|x-y\|\]
\end{enumerate}

\subsection{Main Results}

\begin{lemma}[Gradient Difference]
Under assumptions (A1)-(A4), for any $y \in S_\epsilon(x)$:
\begin{equation}
    \|\nabla_\theta L_{\text{ssl}}(\theta,y) - \nabla_\theta L_{\text{ssl}}(\theta,x)\| \leq K\epsilon
\end{equation}
where $K = 2\beta(2+\delta)$.
\end{lemma}

\begin{proof}
For unit vectors $u(\theta), v(\theta)$:
\begin{equation}
    \nabla_\theta \cos(u,v) = \nabla_\theta(u^T v) - \frac{1}{2}(u^T v)(\nabla_\theta(u^T u) + \nabla_\theta(v^T v))
\end{equation}

By smoothness of $f_\theta$ and the chain rule:
\[\|\nabla_\theta(f_\theta(y)^T f_\theta(T(y))) - \nabla_\theta(f_\theta(x)^T f_\theta(T(x)))\| \leq \beta(2+\delta)\epsilon\]

The normalization terms contribute an additional factor, giving the final bound.
\end{proof}

\begin{theorem}[Influence Separation]
Let $x$ be a point with $I(x) > c$ for some $c > 0$. Then for any $y \in S_\epsilon(x)$:
\begin{equation}
    |I(y) - I(x)| \leq \frac{K\epsilon}{\lambda_{\min}(H)}(2\sqrt{c\lambda_{\max}(H)} + K\epsilon)
\end{equation}
\end{theorem}

\begin{proof}
Let $g_x = \nabla_\theta L_{\text{ssl}}(\theta,x)$ and $g_y = \nabla_\theta L_{\text{ssl}}(\theta,y)$.

By positive definiteness of $H$:
\begin{equation}
    |I(y) - I(x)| = |g_y^T H^{-1} g_y - g_x^T H^{-1} g_x| \leq \frac{1}{\lambda_{\min}(H)}\|g_y + g_x\| \|g_y - g_x\|
\end{equation}

From Lemma 1: $\|g_y - g_x\| \leq K\epsilon$

Since $I(x) = g_x^T H^{-1} g_x > c$:
\[\|g_x\| \leq \sqrt{c\lambda_{\max}(H)}\]

Therefore:
\[\|g_y\| \leq \|g_x\| + \|g_y - g_x\| \leq \sqrt{c\lambda_{\max}(H)} + K\epsilon\]

Combining these bounds gives the result.
\end{proof}


The main theorem shows that points with high influence (>c) must be separated in representation space - their neighborhoods $S_{\epsilon}$ must be small or the influence scores would vary too much.

This explains the t-SNE visualization where high influence points are spread out while low influence points cluster together.



\subsection{Connect influence with setting}
Let $x$ be a point with high influence:
\begin{equation}
    I(x) = -\nabla_\theta L_{\text{ssl}}(\theta,x)^T H^{-1} \nabla_\theta L_{\text{ssl}}(\theta,x) > c
\end{equation}

Consider effect of removing $x$ on any point $z$:

1) SSL effect (view matching):
\begin{equation}
    \Delta L_{\text{ssl}}(z) \approx -\eta \nabla_\theta L_{\text{ssl}}(\theta,z)^T H^{-1} \nabla_\theta L_{\text{ssl}}(\theta,x)
\end{equation}

2) Supervised effect (classification):
\begin{equation}
    \Delta L_{\text{sup}}(z,y) \approx -\eta \nabla_\theta L_{\text{sup}}(\theta,z,y)^T H^{-1} \nabla_\theta L_{\text{ssl}}(\theta,x)
\end{equation}


For high $I(x)$, by definition of cosine similarity in SSL loss:
\begin{equation}
    L_{\text{ssl}}(\theta,x) = 1 - \frac{f_\theta(x)^T f_\theta(T(x))}{\|f_\theta(x)\| \|f_\theta(T(x))\|}
\end{equation}

Large gradient here means: features needed to match views of $x$ are unique to $x$

In downstream supervised eval:
\begin{equation}
    L_{\text{sup}}(\theta,x,y) = -\log \frac{e^{w_y^T f_\theta(x)}}{\sum_k e^{w_k^T f_\theta(x)}}
\end{equation}


\section{Theoretical Analysis}

We provide a theoretical explanation for why removing high-influence points improves SSL training but hurts supervised learning. Our analysis formalizes the intuition that points with high SSL influence tend to be "atypical" examples that lie between clusters, causing tension in representation learning when using cosine similarity. However, these same points are crucial for defining decision boundaries in supervised learning.

\subsection{Setup and Preliminaries}

Let $\mathcal{X} = \mathbb{R}^d$ be our input space. Consider a set of $K$ orthonormal vectors $\{e_1,...,e_K\}$ that define cluster centers. Our data distribution consists of a mixture of "typical" points that lie near cluster centers and "atypical" points that lie between clusters. Formally:

\begin{definition}[Data Distribution]
Let $0 < \rho < \tau < 1$ and $\sigma > 0$ be fixed parameters. The data distribution $\mathcal{D}$ is defined as follows:
\begin{enumerate}
    \item With probability $1-\gamma$, sample a typical point $x \sim p_t$ as:
        \[ x = e_i + \rho\xi \]
        where $i$ is uniform in $[K]$ and $\xi \sim \mathcal{N}(0,I)$
    \item With probability $\gamma$, sample an atypical point $z \sim p_a$ as:
        \[ z = \alpha e_i + \beta e_j + \tau\eta \]
        where $i,j$ are distinct random indices, $\alpha,\beta \geq 0$, $\alpha + \beta = 1$, and $\eta \sim \mathcal{N}(0,I)$
\end{enumerate}

For any point $v$, its augmentation is defined as:
\[ \text{aug}(v) = v + \varepsilon \text{ where } \varepsilon \sim \mathcal{N}(0,\sigma^2I) \]
\end{definition}

Consider an encoder $f_\theta: \mathbb{R}^d \to \mathbb{R}^m$ parameterized by $\theta$. The SSL objective uses cosine similarity between a point and its augmentation. For any two vectors $u,v$, let $L(u,v) = 1 - \cos(u,v)$ denote their cosine distance.

Recall, we define the influence of a point $v$ as:
\begin{definition}[Influence]
The influence of a point $v$ is:
\[ I(v) = -\nabla_\theta L(f_\theta(v), f_\theta(\text{aug}(v)))^T H_\theta^{-1} \nabla_\theta L(f_\theta(v), f_\theta(\text{aug}(v))) \]
where $H_\theta$ is the Hessian of the SSL loss.
\end{definition}

Our analysis requires the following assumptions:

\begin{assumption}[Bounded Hessian]
There exist constants $0 < \lambda < \Lambda$ such that:
\[ \lambda I \leq H_\theta \leq \Lambda I \]
\end{assumption}

\begin{assumption}[Jacobian Regularity]
There exist constants $c_1, c_2 > 0$ such that for all $v$ in the support of $\mathcal{D}$:
\[ c_1 \leq \|\nabla_v f_\theta(v)\| \leq c_2 \]
\end{assumption}

\begin{assumption}[Normalized Embeddings]
For all $v$ in the support of $\mathcal{D}$:
\[ \|f_\theta(v)\| = 1 \]
\end{assumption}

\begin{assumption}[Lipschitz Continuity]
$f_\theta$ is $L$-Lipschitz continuous in the input $v$.
\end{assumption}

Additionally, we require the augmentation noise to be sufficiently small relative to the cluster parameters:
\[ \sigma < \min(\rho,\tau)/C \]
for some constant $C > 0$.

\subsection{Main Results}

We first establish a lemma characterizing the gradient of the cosine distance loss for small perturbations.

\begin{lemma}[Gradient Approximation]
Under Assumptions 3 and 4, for any point $v$ with augmentation noise $\|\text{aug}(v) - v\| \leq \delta$ for sufficiently small $\delta$:
\[ \|\nabla_\theta L(f_\theta(v), f_\theta(\text{aug}(v)))\| = \|\nabla_v f_\theta(v)(\text{aug}(v) - v)\| + O(\|\text{aug}(v) - v\|^2) \]
\end{lemma}

\begin{proof}
By Assumption 3, $\|f_\theta(v)\| = 1$ for all $v$. Using this normalization, the cosine distance gradient is:
\[ \nabla_\theta L(f_\theta(v), f_\theta(\text{aug}(v))) = -\nabla_\theta\langle f_\theta(v), f_\theta(\text{aug}(v))\rangle \]

By Taylor's theorem and Assumption 4 (Lipschitz continuity):
\[ f_\theta(\text{aug}(v)) = f_\theta(v) + \nabla_v f_\theta(v)(\text{aug}(v) - v) + R \]
where the remainder term $R$ satisfies $\|R\| \leq \frac{L}{2}\|\text{aug}(v) - v\|^2$.

Substituting this expansion:
\begin{align*}
\nabla_\theta L &= -\nabla_\theta\langle f_\theta(v), f_\theta(v) + \nabla_v f_\theta(v)(\text{aug}(v) - v) + R\rangle \\
&= -\nabla_\theta\langle f_\theta(v), \nabla_v f_\theta(v)(\text{aug}(v) - v)\rangle + O(\|\text{aug}(v) - v\|^2) \\
&= \|\nabla_v f_\theta(v)(\text{aug}(v) - v)\| + O(\|\text{aug}(v) - v\|^2)
\end{align*}
where the last equality follows from Assumption 3.
\end{proof}

Using this gradient characterization and our assumptions on the Hessian and Jacobian, we can bound the influence for both typical and atypical points:

\begin{theorem}[Influence Bounds]
Under Assumptions 1-4 and for sufficiently small $\sigma$, the expected influence of typical and atypical points satisfies:
\begin{align*}
\lambda(c_1^2(\rho^2 + \sigma^2) - O(\rho^3)) &\leq \mathbb{E}[I(x)] \leq \Lambda(c_2^2(\rho^2 + \sigma^2) + O(\rho^3)) \\
\lambda(c_1^2(\tau^2 + \sigma^2) - O(\tau^3)) &\leq \mathbb{E}[I(z)] \leq \Lambda(c_2^2(\tau^2 + \sigma^2) + O(\tau^3))
\end{align*}
where $x$ is a typical point and $z$ is an atypical point.
\end{theorem}

\begin{proof}
For any point $v$, by Assumption 1 (bounded Hessian):
\[ \frac{1}{\Lambda}\|\nabla_\theta L\|^2 \leq I(v) \leq \frac{1}{\lambda}\|\nabla_\theta L\|^2 \]

By Lemma 1 and Assumption 2 (Jacobian regularity):
\[ c_1\|\text{aug}(v) - v\| - O(\|\text{aug}(v) - v\|^2) \leq \|\nabla_\theta L\| \leq c_2\|\text{aug}(v) - v\| + O(\|\text{aug}(v) - v\|^2) \]

For a typical point $x = e_i + \rho\xi$, the augmentation noise gives:
\[ \mathbb{E}[\|\text{aug}(x) - x\|^2] = \mathbb{E}[\|\varepsilon\|^2] = \rho^2 + \sigma^2 \]

Similarly for an atypical point $z$:
\[ \mathbb{E}[\|\text{aug}(z) - z\|^2] = \tau^2 + \sigma^2 \]

Combining these inequalities and taking expectations yields the desired bounds. The $O(\rho^3)$ and $O(\tau^3)$ terms come from the second-order terms in the gradient approximation.
\end{proof}

\begin{corollary}
Since $\tau > \rho$, for any typical point $x$ and atypical point $z$:
\[ \mathbb{E}[I(z)] \geq \frac{\tau^2}{\rho^2}\mathbb{E}[I(x)] - O(\tau^3) \]
\end{corollary}

This result formalizes our intuition that atypical points have higher influence under the SSL objective. The ratio $\tau^2/\rho^2 > 1$ quantifies how much larger their influence is compared to typical points. This explains why removing high-influence points, which correspond to atypical points between clusters, reduces representation learning tension in SSL.
